Evolve Path Tracer: Early Detection of Malicious Addresses in Cryptocurrency

With the ever-increasing boom of Cryptocurrency, detecting fraudulent behaviors and associated malicious addresses draws significant research effort. However, most existing studies still rely on the full history features or full-fledged address transaction networks, thus cannot meet the requirements of early malicious address detection, which is urgent but seldom discussed by existing studies. To detect fraud behaviors of malicious addresses in the early stage, we present Evolve Path Tracer, which consists of Evolve Path Encoder LSTM, Evolve Path Graph GCN, and Hierarchical Survival Predictor. Specifically, in addition to the general address features, we propose asset transfer paths and corresponding path graphs to characterize early transaction patterns. Further, since the transaction patterns are changing rapidly during the early stage, we propose Evolve Path Encoder LSTM and Evolve Path Graph GCN to encode asset transfer path and path graph under an evolving structure setting. Hierarchical Survival Predictor then predicts addresses' labels with nice scalability and faster prediction speed. We investigate the effectiveness and versatility of Evolve Path Tracer on three real-world illicit bitcoin datasets. Our experimental results demonstrate that Evolve Path Tracer outperforms the state-of-the-art methods. Extensive scalability experiments demonstrate the model's adaptivity under a dynamic prediction setting.

==> table/compare_sota_wo_acc.tex <==
\begin{table*}
    \centering
    \fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
    \caption{Scores of different prediction model.}
    \begin{tabular}{cccccccccccccc}
    \toprule
    \toprule
    \multirow{2}{*}{Type} & \multirow{2}{*}{\makecell{Model\\Name}} & \multicolumn{4}{c}{Hack} & \multicolumn{4}{c}{Ransomware} & \multicolumn{4}{c}{Darknet} \cr
    \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} 
    &\quad  & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$ & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$ & $Prec.$ & $Rec.$ & $F1^E$ & $F1^C$  \cr
    \hline
    \multirow{3}{*}{\makecell{Machine \\ Learning}}
    &DT            &0.347	       &0.137	    &0.197	     &0.197        &0.736	      &0.432	    &0.545	     &0.545	       &0.448   	&0.152	    &0.227	       &0.227\cr
    &RF            &\ud{0.405}   &\ud{0.242}	&\ud{0.303}	 &\ud{0.303}   &0.735	      &\ud{0.436}	&0.547	     &0.547        &0.519   	&0.109   	&0.181	       &0.181\cr
    &XGB           &0.347	       &0.137	    &0.197	     &0.197        &\udb{0.865}   &0.435	    &\ud{0.579}	 &\ud{0.579}   &\ud{0.790}	&\ud{0.191}	&\ud{0.308}	   &\ud{0.308}\cr
    \hline
    \multirow{4}{*}{\makecell{Deep \\ Learning}}
    &GRU           &0.298        &0.438       &0.354 	     &0.354        &0.558	      &0.949	    &0.703	     &0.703	       &0.470	     &0.838   	  &0.603	   &0.603\cr
    &M-LSTM        &\ud{0.418}   &0.272	      &0.328         &0.333        &0.561	      &\udb{0.969}  &0.711	     &0.710        &\ud{0.520}	 &\udb{0.845} &\ud{0.642}  &\ud{0.645}\cr
    &CED	       &0.265        &\ud{0.563}	&\ud{0.360}  &0.360        &\ud{0.617}    &0.960	    &\ud{0.752}  &0.751	       &0.478	     &0.829	      &0.606	   &0.606\cr
    &SAFE          &0.285        &0.438	    &0.271       &0.330            &0.616	      &0.963	    &\ud{0.752}  &\ud{0.752}   &0.508	     &0.838	      &0.632	   &0.632\cr
    \hline
    \multirow{3}{*}{\makecell{Address \\ Graph}}
    &GCN           &\ud{0.329}   &0.658	        &\ud{0.420}  &0.428        &0.564	      &0.936	    &0.700       &0.706        &\ud{0.459}  &0.613	      &0.525	   &0.524\cr
    &Skip-GCN      &0.310        &0.685	        &0.394       &0.427        &0.603         &0.935	    &0.729	     &0.735	       &\ud{0.459}  &0.629	      &\ud{0.531}  &0.530\cr
    &Evolve-GCN    &0.282        &\udb{0.753}	&0.397       &0.390        &\ud{0.613}   &\ud{0.944}  &\ud{0.736}   &\ud{0.746}    &\ud{0.459}  &\ud{0.633}   &0.530	   &\ud{0.533}\cr
    \hline
    \multirow{1}{*}{\makecell{Ours}}
    &Evo. PT       &\udb{0.606}  &0.553	    &\udb{0.551} &\udb{0.576}      &0.735         &0.871	    &\udb{0.795} &\udb{0.798}  &0.626       &0.758	      &\udb{0.685} &\udb{0.685}\cr
    \bottomrule
    \bottomrule
    \end{tabular}\vspace{0cm}
    \label{tab:sota_compare}
\end{table*}

